Validation of Modern JSON Schema: Formalization and Complexity

JSON Schema is the de-facto standard schema language for JSON data. The language went through many minor revisions, but the most recent versions of the language added two novel features, dynamic references and annotation-dependent validation, that change the evaluation model. Modern JSON Schema is the name used to indicate all versions from Draft 2019-09, which are characterized by these new features, while Classical JSON Schema is used to indicate the previous versions. These new "modern" features make the schema language quite difficult to understand, and have generated many discussions about the correct interpretation of their official specifications; for this reason we undertook the task of their formalization. During this process, we also analyzed the complexity of data validation in Modern JSON Schema, with the idea of confirming the PTIME complexity of Classical JSON Schema validation, and we were surprised to discover a completely different truth: data validation, that is expected to be an extremely efficient process, acquires, with Modern JSON Schema features, a PSPACE complexity. In this paper, we give the first formal description of Modern JSON Schema, which we consider a central contribution of the work that we present here. We then prove that its data validation problem is PSPACE-complete. We prove that the origin of the problem lies in dynamic references, and not in annotation-dependent validation. We study the schema and data complexities, showing that the problem is PSPACE-complete with respect to the schema size even with a fixed instance, but is in PTIME when the schema is fixed and only the instance size is allowed to vary. Finally, we run experiments that show that there are families of schemas where the difference in asymptotic complexity between dynamic and static references is extremely visible, even with small schemas.

==> addpropsbl.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "a": 0, "b": null }
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "object",
  "additionalProperties": {"type": "integer"},
  "unevaluatedProperties" : false
}
\end{lstlisting}
\end{querybox}


Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"valid": false,
	"keywordLocation": "",
	"absoluteKeywordLocation": "",
	"instanceLocation": "",
	"errors": [
		{
			"valid": false,
			"error": "Expected: [integer] Found: [null]",
			"keywordLocation": "#/additionalProperties",
			"absoluteKeywordLocation": "#/additionalProperties",
			"instanceLocation": "#/b"
		}
	]
}
\end{lstlisting}
\end{querybox}

\caption{{\qunProps}: Annotations returned by {\BL}, example \ref{ex:addprops}.}
\label{fig:addpropsbl}
\end{figure}





==> addpropshj.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "a": 0, "b": null }
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "object",
  "additionalProperties": {"type": "integer"},
  "unevaluatedProperties" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
...
\end{lstlisting}
\end{querybox}
\caption{{\qunProps}: Annotations returned by {\HJ}, example \ref{ex:addprops}.}
\label{fig:addpropshj}
\end{figure}

==> addpropsje.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "a": 0, "b": null }
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "object",
  "additionalProperties": {"type": "integer"},
  "unevaluatedProperties" : false
}
\end{lstlisting}
\end{querybox}


Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "valid": false,
  "keywordLocation": "",
  "absoluteKeywordLocation": "https://json-everything/base#",
  "instanceLocation": "",
  "errors": [
    {
      "valid": true,
      "keywordLocation": "/additionalProperties",
      "absoluteKeywordLocation": "https://json-everything/base#/additionalProperties",
      "instanceLocation": "/a"
    },
    {
      "valid": false,
      "keywordLocation": "/additionalProperties",
      "absoluteKeywordLocation": "https://json-everything/base#/additionalProperties",
      "instanceLocation": "/b",
      "errors": [],
      {
        "valid": false,
        "keywordLocation": "/additionalProperties/type",
        "absoluteKeywordLocation": "https://json-everything/base#/additionalProperties/type",
        "instanceLocation": "/b",
        "error": "Value is \"null\" but should be \"integer\""
      }
    },
    {
      "valid": false,
      "keywordLocation": "/unevaluatedProperties",
      "absoluteKeywordLocation": "https://json-everything/base#/unevaluatedProperties",
      "instanceLocation": "/b",
      "error": "All values fail against the false schema"
    }
  ]
}
\end{lstlisting}
\end{querybox}

\caption{{\qunProps}: Annotations returned by {\JE}, example \ref{ex:addprops}.}
\label{fig:addpropsje}
\end{figure}


==> addpropsjs.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "a": 0, "b": null }
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "object",
  "additionalProperties": {"type": "integer"},
  "unevaluatedProperties" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
    "valid": false,
    "instanceLocation": "",
    "keywordLocation": "",
    "absoluteKeywordLocation": "urn:uuid:2ca...#",
    "errors": [
        {
            "instanceLocation": "/b",
            "keywordLocation": "/additionalProperties/type",
            "absoluteKeywordLocation": "urn:uuid:2ca...#/additionalProperties/type",
            "error": "The instance must be of type \"integer\""
        },
        {
            "instanceLocation": "",
            "keywordLocation": "/unevaluatedProperties",
            "absoluteKeywordLocation": "urn:uuid:2ca...#/unevaluatedProperties",
            "error": [
                "a",
                "b"
            ]
        }
    ]
}
\end{lstlisting}
\end{querybox}
\caption{{\qunProps}: Annotations returned by {\JSD}, example \ref{ex:addprops}.}
\label{fig:addpropsjs}
\end{figure}

==> addpropske.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "a": 0, "b": null }
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "object",
  "additionalProperties": {"type": "integer"},
  "unevaluatedProperties" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "errors": [
    {
      "error": "got null, not integer",
      "instanceLocation": "/b",
      "keywordLocation": "/additionalProperties/type"
    }
  ],
  "valid": false
}
\end{lstlisting}
\end{querybox}
\caption{{\qunProps}: Annotations returned by {\KE}, example \ref{ex:addprops}.}
\label{fig:addpropsjs}
\end{figure}

==> contbl.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 1, 2, "foo" ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "prefixItems": [false],
  "contains": {"type": "string"},
  "unevaluatedItems": false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"valid": false,
	"keywordLocation": "",
	"absoluteKeywordLocation": "",
	"instanceLocation": "",
	"errors": [
		{
			"valid": false,
			"error": "False",
			"keywordLocation": "#/prefixItems/0",
			"absoluteKeywordLocation": "#/prefixItems/0",
			"instanceLocation": "#/0"
		},
		{
			"valid": false,
			"error": "False",
			"keywordLocation": "#/unevaluatedItems",
			"absoluteKeywordLocation": "#/unevaluatedItems",
			"instanceLocation": "#/1"
		}
	]
}
\end{lstlisting}
\end{querybox}

\caption{{\qcont}: Annotations returned by {\BL}, example \ref{ex:cont}.}
\label{fig:contbl}
\end{figure}


==> contje.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 1, 2, "foo" ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "prefixItems": [false],
  "contains": {"type": "string"},
  "unevaluatedItems": false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "valid": false,
  "keywordLocation": "",
  "absoluteKeywordLocation": "https://json-everything/base#",
  "instanceLocation": "",
  "errors": [
    {
      "valid": false,
      "keywordLocation": "/0",
      "absoluteKeywordLocation": "https://json-everything/base#/0",
      "instanceLocation": "/0",
      "error": "All values fail against the false schema"
    },
    {
      "valid": false,
      "keywordLocation": "/contains",
      "absoluteKeywordLocation": "https://json-everything/base#/contains",
      "instanceLocation": "/0",
      "errors": [],
      {
        "valid": false,
        "keywordLocation": "/contains/type",
        "absoluteKeywordLocation": "https://json-everything/base#/contains/type",
        "instanceLocation": "/0",
        "error": "Value is \"integer\" but should be \"string\""
      }
    },
    {
      "valid": false,
      "keywordLocation": "/contains",
      "absoluteKeywordLocation": "https://json-everything/base#/contains",
      "instanceLocation": "/1",
      "errors": [],
      {
        "valid": false,
        "keywordLocation": "/contains/type",
        "absoluteKeywordLocation": "https://json-everything/base#/contains/type",
        "instanceLocation": "/1",
        "error": "Value is \"integer\" but should be \"string\""
      }
    },
    {
      "valid": true,
      "keywordLocation": "/contains",
      "absoluteKeywordLocation": "https://json-everything/base#/contains",
      "instanceLocation": "/2"
    },
    {
      "valid": false,
      "keywordLocation": "/unevaluatedItems",
      "absoluteKeywordLocation": "https://json-everything/base#/unevaluatedItems",
      "instanceLocation": "/1",
      "error": "All values fail against the false schema"
    }
  ]
}
\end{lstlisting}
\end{querybox}

\caption{{\qcont}: Annotations returned by {\JE}, example \ref{ex:cont}.}
\label{fig:contje}
\end{figure}


==> contjs.tex <==

\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 1, 2, "foo" ]
\end{lstlisting}
\end{querybox}
Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "prefixItems": [false],
  "contains": {"type": "string"},
  "unevaluatedItems": false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
    "valid": false,
    "instanceLocation": "",
    "keywordLocation": "",
    "absoluteKeywordLocation": "urn:uuid:bc389dfd-7f20...#",
    "errors": [
        {
            "instanceLocation": "/0",
            "keywordLocation": "/prefixItems/0",
            "absoluteKeywordLocation": "urn:uuid:bc389dfd-7f20...#/prefixItems/0",
            "error": "The instance is disallowed by a boolean false schema"
        },
        {
            "instanceLocation": "",
            "keywordLocation": "/unevaluatedItems",
            "absoluteKeywordLocation": "urn:uuid:bc389dfd-7f20...#/unevaluatedItems",
            "error": [
                0,
                1
            ]
        }
    ]
}
\end{lstlisting}
\end{querybox}

\caption{{\qcont}: Annotations returned by {\JSD}, example \ref{ex:cont}.}
\label{fig:contjs}
\end{figure}


==> contke.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 1, 2, "foo" ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "prefixItems": [false],
  "contains": {"type": "string"},
  "unevaluatedItems": false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "errors": [
    {
      "error": "item not permitted",
      "instanceLocation": "/0",
      "keywordLocation": "/prefixItems/0"
    },
    {
      "error": "additional item not permitted",
      "instanceLocation": "/1",
      "keywordLocation": "/unevaluatedItems"
    },
    {
      "error": "subschema is not valid against all additional items",
      "instanceLocation": "",
      "keywordLocation": "/unevaluatedItems"
    }
  ],
  "valid": false
}
\end{lstlisting}
\end{querybox}

\caption{{\qcont}: Annotations returned by {\KE}, example \ref{ex:cont}.}
\label{fig:contje}
\end{figure}


==> figures.tex <==
\input{evann.tex}

\input{blann.tex}

\input{jsann.tex}

\input{hjann.tex}

\input{keann.tex}

%%%

\input{addpropsje.tex}

\input{addpropsbl.tex}

\input{addpropsjs.tex}

\input{addpropske.tex}

%%%

\input{pritemje.tex}

\input{pritemsbl.tex}

\input{pritemsjs.tex}

\input{pritemske.tex}

%%%%

\input{itemje.tex}

\input{itemsbl.tex}

\input{itemsjs.tex}

\input{itemke.tex}

%%%

\input{contje.tex}

\input{contbl.tex}

\input{contjs.tex}

\input{contke.tex}

%%

\input{schemaje.tex}

\input{schemabl.tex}

\input{schemajs.tex}

\input{schemake.tex}
%%%

\input{notje.tex}

\input{notje2.tex}

\input{notbl.tex}

\input{notjs.tex}

\input{notke.tex}


==> itemje.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 1, 2, "bar" ]
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "array",
  "items":  { "type": "integer" }, 
  "unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "valid": false,
  "keywordLocation": "",
  "absoluteKeywordLocation": "https://json-everything/base#",
  "instanceLocation": "",
  "errors": [
    {
      "valid": true,
      "keywordLocation": "/items",
      "absoluteKeywordLocation": "https://json-everything/base#/items",
      "instanceLocation": "/0"
    },
    {
      "valid": true,
      "keywordLocation": "/items",
      "absoluteKeywordLocation": "https://json-everything/base#/items",
      "instanceLocation": "/1"
    },
    {
      "valid": false,
      "keywordLocation": "/items",
      "absoluteKeywordLocation": "https://json-everything/base#/items",
      "instanceLocation": "/2",
      "errors": [],
      {
        "valid": false,
        "keywordLocation": "/items/type",
        "absoluteKeywordLocation": "https://json-everything/base#/items/type",
        "instanceLocation": "/2",
        "error": "Value is \"string\" but should be \"integer\""
      }
    }
  ]
}
\end{lstlisting}
\end{querybox}

\caption{{\qits}: Annotations returned by {\JE}, example \ref{ex:items}.}
\label{fig:itemje}
\end{figure}


==> itemke.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 1, 2, "bar" ]
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "array",
  "items":  { "type": "integer" }, 
  "unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "errors": [
    {
      "error": "got string, not integer",
      "instanceLocation": "/2",
      "keywordLocation": "/items/type"
    }
  ],
  "valid": false
}
\end{lstlisting}
\end{querybox}

\caption{{\qits}: Annotations returned by {\KE}, example \ref{ex:items}.}
\label{fig:itemje}
\end{figure}


==> itemsbl.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 1, 2, "bar" ]
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "array",
  "items":  { "type": "integer" }, 
  "unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"valid": false,
	"keywordLocation": "",
	"absoluteKeywordLocation": "",
	"instanceLocation": "",
	"errors": [
		{
			"valid": false,
			"error": "Expected: [integer] Found: [string]",
			"keywordLocation": "#/items",
			"absoluteKeywordLocation": "#/items",
			"instanceLocation": "#/2"
		}
	]
}
\end{lstlisting}
\end{querybox}

\caption{{\qits}: Annotations returned by {\BL}, example \ref{ex:items}.}
\label{fig:itembl}
\end{figure}


==> itemsjs.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 1, 2, "bar" ]
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "type": "array",
  "items":  { "type": "integer" }, 
  "unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
    "valid": false,
    "instanceLocation": "",
    "keywordLocation": "",
    "absoluteKeywordLocation": "urn:uuid:f1c013...#",
    "errors": [
        {
            "instanceLocation": "/2",
            "keywordLocation": "/items/type",
            "absoluteKeywordLocation": "urn:uuid:f1c013...#/items/type",
            "error": "The instance must be of type \"integer\""
        },
        {
            "instanceLocation": "",
            "keywordLocation": "/unevaluatedItems",
            "absoluteKeywordLocation": "urn:uuid:f1c013...#/unevaluatedItems",
            "error": [
                0,
                1,
                2
            ]
        }
    ]
}
\end{lstlisting}
\end{querybox}
\caption{{\qits}: Annotations returned by {\JSD}, example \ref{ex:items}.}
\label{fig:itemsjs}
\end{figure}


==> keann.tex <==
% https://github.com/karenetheridge/JSON-Schema-Modern
% Commit hash 8adc214 

% https://github.com/sdbs-uni-p/ke_validator
% Commit hash 5bc31ec

\begin{figure}[h]
\footnotesize

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "a": 0, "b": 0, "c": 0 }
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/onlya_no_b.json",
  "type": "object",
  "properties":  { 
        "a": {"type": "integer"} ,
        "b": false
  },
  "unevaluatedProperties" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "errors": [
    {
      "absoluteKeywordLocation": "https://formalize.edu/onlya_no_b.json#/properties/b",
      "error": "property not permitted",
      "instanceLocation": "/b",
      "keywordLocation": "/properties/b"
    },
    {
      "absoluteKeywordLocation": "https://formalize.edu/onlya_no_b.json#/unevaluatedProperties",
      "error": "additional property not permitted",
      "instanceLocation": "/c",
      "keywordLocation": "/unevaluatedProperties"
    },
    {
      "absoluteKeywordLocation": "https://formalize.edu/onlya_no_b.json#/unevaluatedProperties",
      "error": "not all additional properties are valid",
      "instanceLocation": "",
      "keywordLocation": "/unevaluatedProperties"
    }
  ],
  "valid": false
}
\end{lstlisting}
\end{querybox}

\caption{Annotations returned by {\KE}, example \ref{ex:vlds}.}
\label{fig:evann}
\end{figure}


==> notbl.tex <==
%0 is NOT evaluated

\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 0 ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"$schema": "https://json-schema.org/draft/2020-12/schema",
	"not" : {
	    "contains" : { "type" : "integer"}
	},
	"unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"valid": false,
	"keywordLocation": "",
	"absoluteKeywordLocation": "",
	"instanceLocation": "",
	"errors": [
		{
			"valid": false,
			"error": "Not condition passed",
			"keywordLocation": "",
			"absoluteKeywordLocation": "",
			"instanceLocation": "\#"
		},
		{
			"valid": false,
			"error": "False",
			"keywordLocation": "\#/unevaluatedItems",
			"absoluteKeywordLocation": "\#/unevaluatedItems",
			"instanceLocation": "\#/0"
		}
	]
}
\end{lstlisting}
\end{querybox}

\caption{Annotations out of $\qnot$: annotations returned by {\BL}.}
\label{fig:notbl}
\end{figure}


==> notbl2.tex <==
%0 is NOT evaluated, neither is 1

begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 0 ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"$schema": "https://json-schema.org/draft/2020-12/schema",
	"not" : {
	    "contains" : { "type" : "integer"}
	},
	"unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"valid": false,
	"keywordLocation": "",
	"absoluteKeywordLocation": "",
	"instanceLocation": "",
	"errors": [
		{
			"valid": false,
			"error": "Not condition passed",
			"keywordLocation": "",
			"absoluteKeywordLocation": "",
			"instanceLocation": "\#"
		},
		{
			"valid": false,
			"error": "False",
			"keywordLocation": "\#/unevaluatedItems",
			"absoluteKeywordLocation": "\#/unevaluatedItems",
			"instanceLocation": "\#/0"
		},
		{
			"valid": false,
			"error": "False",
			"keywordLocation": "\#/unevaluatedItems",
			"absoluteKeywordLocation": "\#/unevaluatedItems",
			"instanceLocation": "\#/1"
		}
	]
}
\end{lstlisting}
\end{querybox}

\caption{Annotations out of $\qnot$:Annotations returned by {\BL}, example \ref{ex:nottwo}.}
\label{fig:notbl}
\end{figure}


==> notje.tex <==
%same as us: 0 evaluated

\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 0 ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"$schema": "https://json-schema.org/draft/2020-12/schema",
	"not" : {
	    "contains" : { "type" : "integer"}
	},
	"unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "valid": false,
  "evaluationPath": "",
  "schemaLocation": "https://json-everything.net/016227154c",
  "instanceLocation": "",
  "details": [
    {
      "valid": true,
      "evaluationPath": "/not",
      "schemaLocation": "https://json-everything.net/016227154c#/not",
      "instanceLocation": "",
      "annotations": {
        "contains": [
          0
        ]
      },
      "details": [
        {
          "valid": true,
          "evaluationPath": "/not/contains",
          "schemaLocation": "https://json-everything.net/016227154c#/not/contains",
          "instanceLocation": "/0"
        }
      ]
    }
  ]
}
\end{lstlisting}
\end{querybox}

\caption{Annotations out of $\qnot$: annotations returned by {\JE}.}
\label{fig:notje}
\end{figure}


==> notje2.tex <==
%0 is evaluated 1 is not

\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 0, "foo" ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"$schema": "https://json-schema.org/draft/2020-12/schema",
	"not" : {
	    "contains" : { "type" : "integer"}
	},
	"unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "valid": false,
  "evaluationPath": "",
  "schemaLocation": "https://json-everything.net/2a3a3e8b34",
  "instanceLocation": "",
  "details": [
    {
      "valid": true,
      "evaluationPath": "/not",
      "schemaLocation": "https://json-everything.net/2a3a3e8b34#/not",
      "instanceLocation": "",
      "annotations": {
        "contains": [
          0
        ]
      },
      "details": [
        {
          "valid": true,
          "evaluationPath": "/not/contains",
          "schemaLocation": "https://json-everything.net/2a3a3e8b34#/not/contains",
          "instanceLocation": "/0"
        },
        {
          "valid": false,
          "evaluationPath": "/not/contains",
          "schemaLocation": "https://json-everything.net/2a3a3e8b34#/not/contains",
          "instanceLocation": "/1",
          "errors": {
            "type": "Value is \"string\" but should be \"integer\""
          }
        }
      ]
    },
    {
      "valid": false,
      "evaluationPath": "/unevaluatedItems",
      "schemaLocation": "https://json-everything.net/2a3a3e8b34#/unevaluatedItems",
      "instanceLocation": "/1",
      "errors": {
        "": "All values fail against the false schema"
      }
    }
  ]
}
\end{lstlisting}
\end{querybox}

\caption{Annotations out of $\qnot$:Annotations returned by {\JE}, verifying that it does not use the 
moot interpretation, Secton \ref{ex:not}.}
\label{fig:notje}
\end{figure}


==> notjs.tex <==
%Zero NOT evaluated!

\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 0 ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"$schema": "https://json-schema.org/draft/2020-12/schema",
	"not" : {
	    "contains" : { "type" : "integer"}
	},
	"unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
    "valid": false,
    "instanceLocation": "",
    "keywordLocation": "",
    "absoluteKeywordLocation": "urn:uuid:6a1f4c56-9504-4696-86c6-c5516d2955ce#",
    "errors": [
        {
            "instanceLocation": "",
            "keywordLocation": "/not",
            "absoluteKeywordLocation": "urn:uuid:6a1f4c56-9504-4696-86c6-c5516d2955ce#/not",
            "error": "The instance must not be valid against the subschema"
        },
        {
            "instanceLocation": "",
            "keywordLocation": "/unevaluatedItems",
            "absoluteKeywordLocation": "urn:uuid:6a1f4c56-9504-4696-86c6-c5516d2955ce#/unevaluatedItems",
            "error": [
                0
            ]
        }
    ]
}
\end{lstlisting}
\end{querybox}

\caption{Annotations out of $\qnot$: annotations returned by {\JS}.}
\label{fig:notjs}
\end{figure}


==> notjs2.tex <==
%None is evaluated!!!

\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 0, "foo" ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"$schema": "https://json-schema.org/draft/2020-12/schema",
	"not" : {
	    "contains" : { "type" : "integer"}
	},
	"unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
    "valid": false,
    "instanceLocation": "",
    "keywordLocation": "",
    "absoluteKeywordLocation": "urn:uuid:023ec2c3-6ba5-4850-af73-2d6130744191#",
    "errors": [
        {
            "instanceLocation": "",
            "keywordLocation": "/not",
            "absoluteKeywordLocation": "urn:uuid:023ec2c3-6ba5-4850-af73-2d6130744191#/not",
            "error": "The instance must not be valid against the subschema"
        },
        {
            "instanceLocation": "",
            "keywordLocation": "/unevaluatedItems",
            "absoluteKeywordLocation": "urn:uuid:023ec2c3-6ba5-4850-af73-2d6130744191#/unevaluatedItems",
            "error": [
                0,
                1
            ]
        }
    ]
}
\end{lstlisting}
\end{querybox}

\caption{Annotations out of $\qnot$:Annotations returned by {\JS}, example \ref{ex:nottwo}.}
\label{fig:notjs}
\end{figure}


==> notke.tex <==


\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 0 ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"$schema": "https://json-schema.org/draft/2020-12/schema",
	"not" : {
	    "contains" : { "type" : "integer" }
	},
	"unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "errors": [
    {
      "error": "subschema is valid",
      "instanceLocation": "",
      "keywordLocation": "/not"
    }
  ],
  "valid": false
}
\end{lstlisting}
\end{querybox}

\caption{Annotations out of $\qnot$:Annotations returned by {\KE}, Section \ref{ex:not}.}
\label{fig:notjs}
\end{figure}


==> pritemje.tex <==

\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 10, "foo", "bar" ]
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/twointegers.json",
  "type": "array",
  "prefixItems": [ { "type": "integer" } , { "type": "integer" } ],
  "unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}


Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "valid": false,
  "keywordLocation": "",
  "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#",
  "instanceLocation": "",
  "errors": [
    {
      "valid": true,
      "keywordLocation": "/0",
      "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/0",
      "instanceLocation": "/0"
    },
    {
      "valid": false,
      "keywordLocation": "/1",
      "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/1",
      "instanceLocation": "/1",
      "errors": [],
      {
        "valid": false,
        "keywordLocation": "/1/type",
        "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/1/type",
        "instanceLocation": "/1",
        "error": "Value is \"string\" but should be \"integer\""
      }
    },
    {
      "valid": false,
      "keywordLocation": "/unevaluatedItems",
      "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/unevaluatedItems",
      "instanceLocation": "/2",
      "error": "All values fail against the false schema"
    }
  ]
}
\end{lstlisting}
\end{querybox}

\caption{{\qprefIts}: Annotations returned by {\JE}, example \ref{ex:pritem}.}
\label{fig:pritemje}
\end{figure}

==> pritemsbl.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 10, "foo", "bar" ]
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/twointegers.json",
  "type": "array",
  "prefixItems": [ { "type": "integer" } , { "type": "integer" } ],
  "unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}


Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"valid": false,
	"keywordLocation": "https://formalize.edu/twointegers.json",
	"absoluteKeywordLocation": "",
	"instanceLocation": "",
	"errors": [
		{
			"valid": false,
			"error": "Expected: [integer] Found: [string]",
			"keywordLocation": "https://formalize.edu/twointegers.json\#/prefixItems/1",
			"absoluteKeywordLocation": "\#/prefixItems/1",
			"instanceLocation": "\#/1"
		},
		{
			"valid": false,
			"error": "False",
			"keywordLocation": "https://formalize.edu/twointegers.json\#/unevaluatedItems",
			"absoluteKeywordLocation": "\#/unevaluatedItems",
			"instanceLocation": "\#/2"
		}
	]
}
\end{lstlisting}
\end{querybox}

\caption{{\qprefIts}: Annotations returned by {\BL}, example \ref{ex:pritem}.}
\label{fig:pritemsbl}
\end{figure}




==> pritemsjs.tex <==
\begin{figure}
\small
Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 10, "foo", "bar" ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/twointegers.json",
  "type": "array",
  "prefixItems": [ { "type": "integer" } , { "type": "integer" } ],
  "unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
    "valid": false,
    "instanceLocation": "",
    "keywordLocation": "",
    "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#",
    "errors": [
        {
            "instanceLocation": "/1",
            "keywordLocation": "/prefixItems/1/type",
            "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/prefixItems/1/type",
            "error": "The instance must be of type \"integer\""
        },
        {
            "instanceLocation": "",
            "keywordLocation": "/unevaluatedItems",
            "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/unevaluatedItems",
            "error": [
                0,
                1,
                2
            ]
        }
    ]
}
\end{lstlisting}
\end{querybox}

\caption{{\qprefIts}: annotations returned by {\JSD}, example \ref{ex:pritem}.}
\label{fig:pritemsjs}
\end{figure}


==> pritemske.tex <==
\begin{figure}
\small
Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
[ 10, "foo", "bar" ]
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/twointegers.json",
  "type": "array",
  "prefixItems": [ { "type": "integer" } , { "type": "integer" } ],
  "unevaluatedItems" : false
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "errors": [
    {
      "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/prefixItems/1/type",
      "error": "got string, not integer",
      "instanceLocation": "/1",
      "keywordLocation": "/prefixItems/1/type"
    },
    {
      "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/unevaluatedItems",
      "error": "additional item not permitted",
      "instanceLocation": "/2",
      "keywordLocation": "/unevaluatedItems"
    },
    {
      "absoluteKeywordLocation": "https://formalize.edu/twointegers.json#/unevaluatedItems",
      "error": "subschema is not valid against all additional items",
      "instanceLocation": "",
      "keywordLocation": "/unevaluatedItems"
    }
  ],
  "valid": false
}
\end{lstlisting}
\end{querybox}

\caption{{\qprefIts}: annotations returned by {\KE}, example \ref{ex:pritem}.}
\label{fig:pritemsjs}
\end{figure}


==> rules.tex <==
% !TeX root = schemaSemantics.tex




\hide{
\adcomm
\adescr
\adefault
\adefs  -----------
\addefs
\atitle
\aname
\atags
\acomment
\aid
\adid
\adschema
\ada
\addref
\adda
}

\subsection{Terminal type-conditional keywords}\label{sec:typecond}

{The following assertions are defined by a set of two rules: (\key{kw}\TTriv) and (\key{kw}})
(Sections \ref{sec:tuterminal} and \ref{sec:tcterminal});
in the table, the length operator $|J|$ counts the number of characters of a string, the number of fields of an object,
and the number of elements of an array. \kw{names}(J) extracts the names of an object.
When $p$ is a pattern or a format, we use $\rlan{p}$ to indicate 
the corresponding set of strings.

When  \TypeOf(\key{kw}) is \emph{no type} then the assertion does not have the (\key{kw}\TTriv) rule and does not have the condition
$\TypeOf(J) = \TypeOf(\key{kw})$ in the (\key{kw}) rule. \\ 
\medskip


\begin{tabular}{| l | l | l |}
\hline 
assertion \key{kw}:J' & \TypeOf(\key{kw}) & \rkw{cond}(J,\key{kw}:J') \\ \hline 
$\aenum: [J_1,\ldots,J_n]$   & \emph{no type} &  $J \in \Set{J_1,\ldots,J_n}$ \\ \hline
$\aconst: J_c $  & \emph{no type} &  $J = J_c$ \\ \hline
$\atype: \rkw{Tp}$ & \emph{no type} &   $\TypeOf(J)= \rkw{Tp}$ \\ \hline
$\atype: [\rkw{Tp}_1,\ldots,\rkw{Tp}_n]$  & \emph{no type} &   $\TypeOf(J) \in \Set{\rkw{Tp}_1,\ldots,\rkw{Tp}_n}$ \\ \hline
\aexmin: q   &  \rnumber &  $J > q$ \\ \hline
\aexmax: q   &  \rnumber &  $J < q$ \\ \hline
\amin: q   &  \rnumber &  J $\geq$ q \\ \hline
\amax: q   &  \rnumber &  J $\leq$ q \\ \hline
\amof: q   &  \rnumber &  $\exists i\in\Int.\ J = i\times q$ \\ \hline
\apatt: p  &  \rstr &  $J \in \rlan{p}$ \\ \hline
\aminL: i   &  \rstr &  $|J| \geq i$ \\ \hline
\amaxL: i   &  \rstr &  $|J| \leq i$ \\ \hline
%\areq: k   &  \robject &  $J = \{ k : J_0, k_1:J_1,\ldots, k_n:J_n \}  $ \\ \hline
%$\apropN : S$  & \robject &    \ldots \\ \hline
\aminP: i  & \robject &  $|J| \geq i$  \\ \hline
\amaxP: i  & \robject &  $|J| \leq i$   \\ \hline
$\areq: \JArr{k_1,\ldots,k_n}$  & \robject &  $\forall i.\ k_i\in \kw{names}(J)$   \\ \hline
\auniqIt: \xtrue  & \rarray &  $J=[J_1,\ldots,J_n]\mbox{\ with\ } n\geq 0 $  \\ 
&&  $\And\ \forall i,j.\ 1 \leq i\neq j \leq n \Implies J_i\neq J_j  $  \\ 
\hline
\auniqIt: \xfalse  & \rarray & T  \\ 
\hline
\aminIt: i  & \rarray &  $|J| \geq i$    \\ \hline
\amaxIt: i  & \rarray &  $|J| \leq i$  \\ \hline
\aformat: \key{format}  & \rstr &  $J \in \rlan{\key{format}}  $  \\ \hline
$\adepR:$
      &  &  $\forall i\in\SetTo{n}.\ $  \\ 
 $\quad\JObjOpen\  k_1: \JArr{k^1_1,\ldots,k^1_{o_1}}$ &\robject  & $\qquad k_i \in   \kw{names}(J)$  \\ 
 $\quad\ \ \ldots,k_n: \JArr{k^n_1,\ldots,k^n_{o_n}}\ \JObjClose$ & & $\qquad \Implies \Set{k^i_1,\ldots,k^i_{o_i}} \subseteq \kw{names}(J)$ \\ \hline
\end{tabular}


\infrule[\key{kw}\TTriv]
{
\TypeOf(J) \neq \TypeOf(\key{kw})
}
{\KJudgCJ{\key{kw}:J'}
 \Ret{T}
 \key{kw}\TTriv(\_)
}

\infrule[\key{kw}]
{
\TypeOf(J) = \TypeOf(\key{kw}) \andalso
r = \rkw{cond}(J,\key{kw}\!:\!J')
}
{\KJudgCJ{\key{kw}\!:\!J'}
 \Ret{r}
 \key{kw}(\_)
}

\hide{
\subsection{Terminal unconditional assertions}

\medskip
\begin{tabular}{| l | l |}
\hline 
assertion \akw{kw}:J'  & \rkw{cond}(J,\akw{kw}:J') \\ \hline 
$\aenum: [J_1,\ldots,J_n]$   &   $J \in \Set{J_1,\ldots,J_n}$ \\ \hline
$\aconst: J_c $  &  $J = J_c$ \\ \hline
$\atype: \rkw{Tp}$ &   $\TypeOf(J)= \rkw{Tp}$ \\ \hline
$\atype: [\rkw{Tp}_1,\ldots,\rkw{Tp}_n]$  &   $\TypeOf(J) \in \Set{\rkw{Tp}_1,\ldots,\rkw{Tp}_n}$ \\ \hline
\end{tabular}

\infrule[\rkw{kw}]
{
\TypeOf(J) = \TypeOf(\akw{kw}) \andalso
r = \rkw{cond}(J,\akw{kw}\!:\!J')
}
{\KJudgCJ{\akw{kw}\!:\!J'}
 \Ret{r}
 \rkw{kw}(\_)
}
}

\newcommand{\CP}[1]{C^+_{#1}}
\renewcommand{\CP}[1]{C}


\subsection{The boolean applicators}

\infrule[\rany]
{
\forall i\in \SetTo{n}.\ \ \SJudg{\CP{.,i}}{J}{S_i}\Ret{r_i}{\ps_i} \andalso
r=\Or(\SetIIn{r_i}{i}{\SetTo{n}}) 
}
{\KJudg{C}{J}{\aany:[S_1,...,S_n]}
 \Ret{r}
 \rany(\_,\pList{\ps_1,\ldots,\ps_n})
}


\infrule[\rall]
{
\forall i\in \SetTo{n}.\ \SJudg{\CP{.,i}}{J}{S_i}\Ret{r_i}{\ps_i} \andalso
r=\And(\SetIIn{r_i}{i}{\SetTo{n}}) 
}
{\KJudgCJ{\aall:[S_1,...,S_n]}
 \Ret{r}
 \rall(\_,\pList{\ps_1,\ldots,\ps_n})
}

\infrule[\rone]
{
\forall i\in \SetTo{n}.\ \SJudg{\CP{.,i}}{J}{S_i}\Ret{r_i}{\ps_i} \andalso
r = (\ |\SetST{i}{r_i=T}| = 1 \ )
}
{\KJudgCJ{\aone:[S_1,...,S_n]}
 \Ret{r}
 \rone(\_,\pList{\ps_1,\ldots,\ps_n})
}


\infrule[\rnot]
{
\SJudg{\CP{.,.}}{J}{S}\Ret{r}{\ps} 
}
{\KJudgCJ{\anot:S}
 \Ret{\Not r}
 \rnot(\_,\ps)
}

\subsection{References}

\infrule[\rdref]
{
%S = \Load(\key{absURI}) \andalso
S' = \Get(\Load(\key{absURI}),\key{f}) \andalso
%\SJudg{L  + \key{absURI},\ I,\ \key{absURI}\cat\qkw{\#}\cat\key{f},\ R\cat\QQ/\rdref\QQ}{J}{S'}\Ret{r}{\ps}
\SJudg{C  + \key{absURI}\ }{J}{S'}\Ret{r}{\ps}
}
{%\SJudg{L,I,A,R}{J}{\adref: \key{absURI}\cat\qkw{\#}\cat\key{f}}
 \KJudg{C}{J}{\adref: \key{absURI}\cat\qkw{\#}\cat\key{f}}
 \Ret{r}
 \rdref(\_,\ps)
}

\infrule[\rddref]
{
\DGet(\Load(\key{absURI}),\key{f}) \neq \bot  \andalso
\key{fURI} = \fstURI(C,f) \\[\NL]
S' = \DGet(\Load(\key{fURI}),\key{f}) \andalso
%\SJudg{L  + \key{fURI},\ I,\ \key{fURI}\cat\qkw{\#}\cat\key{f},\ R\cat\QQ/\rdref\QQ}{J}{S'}\Ret{r}{\ps}
\SJudg{C  + \key{fURI}\ }{J}{S'}\Ret{r}{\ps}
}
{%\SJudg{L,I,A,R}{J}{\addref: \key{absURI}\cat\qkw{\#}\cat\key{f}}
 \KJudg{C}{J}{\addref: \key{absURI}\cat\qkw{\#}\cat\key{f}}
 \Ret{r}
 \rddref(\_,\ps)
}

\infrule[\rddref\rkw{AsRef}]
{
\DGet(\Load(\key{absURI}),\key{f}) = \bot  \\[\NL]
S' = \Get(\Load(\key{absURI}),\key{f}) \andalso
%\SJudg{L  + \key{absURI},\ I,\ \key{absURI}\cat\qkw{\#}\cat\key{f},\ R\cat\QQ/\rddref\QQ}{J}{S'}\Ret{r}{\ps}
\SJudg{C  + \key{absURI}\ }{J}{S'}\Ret{r}{\ps}
}
{%\SJudg{L,I,A,R}{J}{\addref: \key{absURI}\cat\qkw{\#}\cat\key{f}}
 \KJudg{C}{J}{\addref: \key{absURI}\cat\qkw{\#}\cat\key{f}}
  \Ret{r}
 \rddref\rkw{AsRef}(\_,\ps)
}


\subsection{Object and array applicators: independent applicators}\label{sec:indeprules}

The following assertions are defined by a set of two rules: (\key{kw}\TTriv) and (\key{kw});
the (\key{kw}\TTriv) rules are specified by the following table; the  (\key{kw}) rules are specified after the table.

\medskip

\begin{tabular}{| l | l | l |}
\hline 
assertion $\key{kw}:J'$ & $\TypeOf(\key{kw})$  \\ \hline 
%$\aprops : \JObj{ f : S }$  & \robject   \\ \hline
$\apattProps: \JObj{ p_1 : S_1,\ldots,p_m : S_m }$  & \robject   \\ \hline
$\aprops: \JObj{ k_1 : S_1,\ldots,k_m : S_m }$  & \robject   \\ \hline
$\apropN: S$  & \robject   \\ \hline
$\aprefIts: S$  & \rarray   \\ \hline
$\acont: S$  & \rarray   \\ \hline
$\adepS:  \JObj{k_1: S_1,\ldots,k_n:S_n}$  & \robject   \\ \hline
\end{tabular}


\infrule[\rpattProps]
{
J = \JObj{k'_1:J_1,\ldots,k'_n:J_n} \andalso
\Set{(i_1,j_1),\ldots,(i_l,j_l)} = \SetST{(i,j)}{k'_i \in \rlan{p_j}} \\[\NL]
\forall q\in \SetTo{l}.\ 
\SJudg{\CP{k'_{i_q},k_{j_q}}}{J_{i_q}}{S_{j_q}}\Ret{r_q}{\ps_q} \andalso
r=\And(\SetIIn{r_q}{q}{\SetTo{l}}) 
}
{
\KJudgCJ{\apattProps: \JObj{ p_1 : S_1,\ldots,p_m : S_m }} 
\qquad\qquad\qquad\qquad\qquad\qquad\qquad
\\[\NL]
 \qquad\qquad\qquad\qquad\qquad\qquad\qquad
 \Ret{r}
 {\rpattProps(\_,\pList{(k'_{i_1},p_{j_1}),\ldots,(k'_{i_l},p_{j_l})},\pList{\ps_1,\ldots,\ps_l})}
}

\infrule[\rprops]
{
J = \JObj{k'_1:J_1,\ldots,k'_n:J_n} \andalso
\Set{(i_1,j_1),\ldots,(i_l,j_l)} = \SetST{(i,j)}{k'_i=k_j} \\[\NL]
\forall q\in \SetTo{l}.\ 
\SJudg{\CP{k'_{i_q},k_{j_q}}}{J_{i_q}}{S_{j_q}}\Ret{r_q}{\ps_q} \andalso
r=\And(\SetIIn{r_q}{q}{\SetTo{l}})
}
{
\KJudgCJ{\aprops: \JObj{ k_1 : S_1,\ldots,k_m : S_m }} 
\qquad\qquad\qquad\qquad\qquad\qquad\qquad
\\[\NL]
 \qquad\qquad\qquad\qquad\qquad\qquad\qquad
 \Ret{r}
 {\rprops(\_,\pList{(k'_{i_1},k_{j_1}),\ldots,(k'_{i_l},k_{j_l})},\pList{\ps_1,\ldots,\ps_l})}
}

\infrule[\rpropN]
{
J = \JObj{k_1:J_1,\ldots,k_n:J_n} \andalso
\forall i\in \SetTo{n}.\ 
\SJudg{\CP{k_i,.}}{k_i}{S}\Ret{r_i}{\ps_i} \andalso
r=\And(\SetIIn{r(\ps_i)}{i}{\SetTo{n}}) 
}
{
\KJudgCJ{\apropN:S}\Ret{r}
 {\rpropN(\_,\pList{\ps_1,\ldots,\ps_n})}
}


\infrule[\rprefIts]
{
J = \JArr{J_1,\ldots,J_m} \andalso
\forall i\in \SetTo{\Min(n,m)}.\ \SJudg{\CP{i,i}}{J_i}{S_i}\Ret{r_i}{\ps_i} \andalso
r=\And(\SetIIn{r_i}{i}{\SetTo{\Min(n,m)}}) 
}
{\KJudgCJ{\aprefIts: \JArr{S_1,\ldots,S_n}}
 \Ret{r}
 \rprefIts(\_,\pList{\ps_1,\ldots,\ps_{\Min(n,m)}})
}


\infrule[\rcont]
{
J = [J_1,\ldots,J_n] \andalso
\forall i\in \SetTo{n}.\ \SJudg{\CP{i,.}}{J_i}{S}\Ret{r_i}{\ps_i} \andalso
r=\Or(\SetIIn{r_i}{i}{\SetTo{n}}) 
}
{\KJudgCJ{\acont: S}
 \Ret{r}
 \rcont(\_,\pList{\ps_1,\ldots,\ps_n})
}



\infrule[\rdepS]
{
J = \JObj{k'_1: J_1,\ldots,\, k'_m: J_m} \andalso
\Set{i_1,\ldots,i_l} = \SetST{i}{i\in\SetTo{n},\ k_i \in \Set{k'_1,\ldots,\, k'_m}}\\[\NL]
\forall q\in\SetTo{l}.\ 
                       \SJudg{\CP{.,k_{i_q}}}{J}{S_{i_q}}\Ret{r_q}{\ps_q}\andalso
r=\And(\SetIIn{r_q}{q}{\SetTo{l}}) 
}
{\KJudgCJ{\adepS: \JObj{k_1: S_1,\ldots,k_n: S_n}}
\qquad\qquad\qquad\qquad\qquad\qquad\qquad
\\[\NL]
 \qquad\qquad\qquad\qquad\qquad\qquad\qquad
 \Ret{r}
 \rdepS(\_,\pList{k_{i_1},\ldots k_{i_l}},\pList{\ps_1,\ldots,\ps_l})
}

\hide{ OLD VERSION
\infrule[\rdepR]
{
J = \JObj{k'_1: J_1,\ldots,\, k'_m: J_m} \andalso
\Set{i_1,\ldots,i_l} = \SetST{i}{i\in\SetTo{n},\ k_i \in \Set{k'_1,\ldots,\, k'_m}}\\[\NL]
\forall q\in\SetTo{l}.\ 
r_q = ( \forall j\in \SetTo{o_q}.\ k^p_j \in \Set{k'_1,\ldots,\, k'_m} \andalso
r=\And(\SetIIn{r_q}{q}{\SetTo{l}})
}
{\KJudgCJ{\adepR: \JObj{k_1: \JArr{k^1_1,\ldots,k^1_{o_1}},\ldots,k_n: \JArr{k^n_1,\ldots,k^n_{o_n}}}}
\qquad\qquad\qquad\qquad
\\[\NL]
 \qquad\qquad\qquad\qquad
 \Ret{r}
 \rdepR(\_,\pList{k_{i_1},\ldots k_{i_l}},\pList{r_1,\ldots,r_l})   
}
}

\subsection{Dependent keywords}


The following assertions are defined by a set of two rules: (\key{kw}\TTriv) and (\key{kw});
the (\key{kw}\TTriv) rule is specified by the following table.
\medskip

\begin{tabular}{| l | l | l |}
\hline 
assertion $\key{kw}:J'$ & $\TypeOf(\key{kw})$  \\ \hline 
$\aunProps: S$  & \robject   \\ \hline
$\aaddProps: S$  & \robject   \\ \hline
$\aunIts: S$  & \rarray   \\ \hline
$\ait: S$  & \rarray   \\ \hline
$\aminC: i$  & \rarray   \\ \hline
$\amaxC: i$  & \rarray   \\ \hline
\end{tabular}


\infrule[\runProps]
{
J=\JObj{k_1 : J_1,\ldots,k_n:J_n} \andalso
\KLJudgCJ{\Kl}\Ret{\rl}{\pkl} \\[\NL]
%\Set{k_{i_1},\ldots,k_{i_l}} = \Set{k_1,\ldots,k_n} \setminus \EvalProps(\pkl) \\[\NL]
\Set{{i_1},\ldots,{i_l}} = \SetST{i}{1\leq i \leq n \And\ k_i \not\in \EvalProps(\pkl)} \\[\NL]
\forall q\in \SetTo{l}.\ 
\SJudg{\CP{k_{i_q},.}}{J_{i_q}}{S}\Ret{r_q}{\ps_q} \andalso
r=\And(\SetIIn{r_q}{q}{\SetTo{l}}) 
}
{
\KLJudgCJ{(\Kl\plus\aunProps : S)}
\qquad\qquad\qquad\qquad
\\[\NL]
 \qquad\qquad\qquad\qquad
 \Ret{\rl\plus r}{\pkl\plus\runProps(\_,\pList{k_{i_1}\ldots,k_{i_l}},\pList{\ps_1,\ldots,\ps_l})}
}

\infrule[\raddProps]
{
J=\JObj{k_1 : J_1,\ldots,k_n:J_n} \andalso
\KLJudgCJ{\Kl}\Ret{\rl}{\pkl} \\[\NL]
%\Set{k_1,\ldots,k_n} \setminus \EvalProps(\pkl) = \Set{k_{i_1},\ldots,k_{i_m}} \\[\NL]
\Set{{i_1},\ldots,{i_l}} = \SetST{i}{1\leq i \leq n \And\ k_i \not\in \AdjEvalProps(\pkl)} \\[\NL]
\forall q\in \SetTo{l}.\ 
\SJudg{\CP{k_{i_q},.}}{J_{i_q}}{S}\Ret{r_q}{\ps_q} \andalso
r=\And(\SetIIn{r_q}{p}{\SetTo{l}})  
}
{
\KLJudgCJ{(\Kl\plus\aaddProps : S)}
\qquad\qquad\qquad\qquad
\\[\NL]
 \qquad\qquad\qquad\qquad
 \Ret{\rl\plus r}{\pkl\plus\raddProps(\_,\pList{k_{i_1}\ldots,k_{i_l}},\pList{\ps_1,\ldots,\ps_l})}
}

\infrule[\runIts]
{
J=\JArr{J_1,...,J_n} \andalso
\KLJudgCJ{\Kl}\Ret{\rl}{\pkl} \andalso
\Set{i_1,\ldots,i_l} = \SetTo{n} \setminus \EvalItems(\pkl) \\[\NL]
\forall q\in \SetTo{l}.\ \SJudg{\CP{i_q,.}}{J_{i_q}}{S}\Ret{r_q}{\ps_q} \andalso
r=\And(\SetIIn{r_q}{q}{\SetTo{l}}) 
}
{\KLJudgCJ{(\Kl\plus\aunIts : S)}
\Ret{\rl\plus r}{\pkl\plus\runIts(\_,\pList{i_1\ldots,i_l},\pList{\ps_1,\ldots,\ps_l})}
}

\infrule[\rits]
{
J=\JArr{J_1,...,J_n} \andalso
\KLJudgCJ{\Kl}\Ret{\rl}{\pkl} \andalso
\Set{i_1,\ldots,i_l} = \SetTo{n} \setminus \AdjEvalItems(\pkl) \\[\NL]
\forall q\in \SetTo{l}.\ \SJudg{\CP{i_q,.}}{J_{i_q}}{S}\Ret{r_q}{\ps_q} \andalso
r=\And(\SetIIn{r_q}{q}{\SetTo{l}}) 
}
{\KLJudgCJ{(\Kl\plus\aits : S)}
\Ret{\rl\plus r}{\pkl\plus\rits(\_,\pList{i_1\ldots,i_l},\pList{\ps_1,\ldots,\ps_l})}
}


\infrule[\rmaxC]
{
J=\JArr{J_1,...,J_n} \andalso
\KLJudgCJ{\Kl}\Ret{\rl}{\pkl} \\[\NL]
 \rcont(\_,\pList{\ps_1,\ldots,\ps_n}) \in \pkl \andalso
r = (\ |\SetST{\ps_j}{r(\ps_j)=T} | \leq i\ )
}
{\KLJudgCJ{(\Kl\plus\amaxC : i)}
\Ret{\rl\plus r}{\pkl\plus\rmaxC(\_)}
}

\infrule[\rminC\rkw{-non-0}]
{
i > 0 \andalso
J=\JArr{J_1,...,J_n} \andalso
\KLJudgCJ{\Kl}\Ret{\rl}{\pkl}  \\[\NL]
 \rcont(\_,\pList{\ps_1,\ldots,\ps_n}) \in \pkl \andalso
r = (\ |\SetST{\ps_j}{r(\ps_j)=T} | \geq i\ )
}
{\KLJudgCJ{(\Kl\plus\aminC : i)}
\Ret{\rl\plus r}{\pkl\plus\rminC\rkw{-non-0}(\_)}
}

\infrule[\rminC\rkw{-0}]
{
J=\JArr{J_1,...,J_n} \andalso
%\KLJudg{C^+}{J}{\Kl}\Ret{\rl}{( \pkl_0 \plus \rcont(C,J,K,r,\psl) )}
\KLJudg{C^+}{J}{\Kl\plus\acont : S}\Ret{\rl+r_c}{\pkl\plus \rcont(C_c,J,K_c,r_c,\psl_c) )}
}
{
\KLJudgCJ{\Kl\plus\acont : S\plus\aminC : 0}
\qquad\qquad\qquad\qquad
 \\[\NL]
 \qquad\qquad\qquad\qquad
  \Ret{\rl\plus T\plus T}
  {\pkl \plus \rcont(C_c,J,K_c,T,\psl_c) \plus \rminC\rkw{-0}(\_)
  }
}

\infrule[\rklist-(n+1)]
{
k:J'\in\key{IndKeyOrT} \andalso
\KLJudgCJ{\Kl}\Ret{\rl}{\pkl} \andalso
\KJudg{C}{J}{K}\Ret{r}{\pk} \\[\NL]
%\mbox{where\ \ \ }
%C_K^+.A = C.A\cat\qqs\cat k \andalso
%\RAsA{K}  \andalso
%C_K^+.I = C.I \andalso
%C_K^+.L = C.L  
}
{\KLJudgCJ{(\Kl\plus K)}
\Ret{\rl\plus r}{\pkl\plus\pk}
}

\hide{
\infrule[\rklist-(n+1)]
{
k:J'\ \mbox{is irrelevant for validation} \andalso
\KLJudgCJ{\Kl}\Ret{\rl}{\pkl} \andalso
}
{\KLJudgCJ{(\Kl\plus k : J')}
\Ret{\rl\plus r}{\pkl\plus\pk}
}
}

\infax[\rklist-0]
{\KLJudgCJ{\List{}}
 \Ret{\List{}}{\List{}}
}




\subsection{If-then-else}\label{sec:iterulescomplete}

\infrule[\rkw{if-true-then}]
{
\KLJudg{C}{J}{\Kl}\Ret{\rl}{\pkl} \andalso
\SJudg{\CP{.,.}}{J}{S_i}\Ret{T}{\ps_i} \andalso
\SJudg{\CP{.,.}}{J}{S_t}\Ret{r_t}{\ps_t}
}
{
\KLJudgCJ{(\ \Kl\plus 
  \aif: S_i \plus
  \athen: S_t \ (\plus
  \aelse: S_e)^?\ )}
  \RetL{\rl \plus T \plus r_t}{\pkl\plus\rif(\_,\ps_i)\plus\rthen(\_,\ps_t)}
}

\infrule[\rkw{if-true-no-then}]
{
\KLJudg{C}{J}{\Kl}\Ret{\rl}{\pkl} \andalso
\SJudg{\CP{.,.}}{J}{S_i}\Ret{T}{\ps_i}
}
{
\KLJudgCJ{(\ \Kl\plus 
  \aif: S_i
  \ (\plus
  \aelse: S_e)^?\ )}
  \RetL{\rl \plus T}{\pkl\plus\rif(\_,\ps_i)}
}


\infrule[\rkw{if-false-else}]
{
\KLJudg{C}{J}{\Kl}\Ret{\rl}{\pkl} \andalso
\SJudg{\CP{.,.}}{J}{S_i}\Ret{F}{\ps_i} \andalso
\SJudg{\CP{.,.}}{J}{S_e}\Ret{r_e}{\ps_e}
}
{
\KLJudgCJ{(\ \Kl\plus 
  \aif: S_i  
  \ (\plus \athen: S_t \ )^?
  \ \plus \aelse: S_e)}
  %\Ret{\rl \plus F \plus r_e}{\pkl\plus\rif(\_,\ps_i)\plus\relse(\_,\ps_e)}
  \RetL{\rl \plus T \plus r_e}{\pkl\plus\rif(\_,\ps_i)\plus\relse(\_,\ps_e)}
}

\infrule[\rkw{if-false-no-else}]
{
\KLJudg{C}{J}{\Kl}\Ret{\rl}{\pkl} \andalso
\SJudg{\CP{.,.}}{J}{S_i}\Ret{F}{\ps_i}
}
{
\KLJudgCJ{(\ \Kl\plus 
  \aif: S_i 
  \ (\plus \athen: S_t \ )^?\ )
  }
%  \Ret{\rl \plus F}{\pkl\plus\rif(\_,\ps_i)}
  \RetL{\rl \plus T}{\pkl\plus\rif(\_,\ps_i)}
}

\subsection{The trivial rule}


\infrule[\mbox{\em kw}-\rkw{trivial}]
{
kw \in \key{Other}
}
{\KJudgCJ{kw : J'}
 \Ret{T}
 {kw}(\_)
}

\subsection{Schema rules}


\infrule[\rtrueS]
{
}
{\SJudgCJ{\atrue}
 \Ret{T}
 \rtrueS(\_)
}

\infrule[\rfalseS]
{
}
{\SJudgCJ{\afalse}
 \Ret{F}
 \rfalseS(\_)
}


\infrule[\rschema]
{
\forall \key{absURI}.\ ( K_1 \neq \qdid : \key{absURI}) \\
\KLJudgCJ{\List{K_1,\ldots,K_n}}\RetL{\List{r_1,\ldots,r_n}}{\List{\pk_1,\ldots,\pk_n}} \andalso
r=\And(\SetIIn{r(\pk_i)}{i}{\SetTo{n}}) 
}
{\SJudgCJ{\JObj{K_1,\ldots,K_n}}
 \Ret{r}
 \rschema(\_,\pList{\pk_1,\ldots,\pk_n})
}

\infrule[\rschema\rkw{\$id}]
{
\KLJudg{C+\key{absURI}}{J}{\List{K_1,\ldots,K_n}}\RetL{\List{r_1,\ldots,r_n}}{\List{\pk_1,\ldots,\pk_n}} \andalso
r=\And(\SetIIn{r(\pk_i)}{i}{\SetTo{n}}) 
}
{\SJudgCJ{\JObj{\qdid: \key{absURI}, K_1,\ldots,K_n}}
 \Ret{r}
 \rschema\rkw{\$id}(\_,\pList{\pk_1,\ldots,\pk_n})
}





\subsection{Rules for $\EvalStar$ and for $\AdjEvalStar$}\label{sec:evalrules}



$$
\begin{array}{llll}
\!\!\!\!\EvalStar(\pk/\ps): \\[\NL]
%\!\!\!\!\EvalStar(\pk): \qquad\qquad\qquad\qquad\qquad\\[\NL]
\multicolumn{1}{l}{
\EvalItems(\rprefIts(\_,\pList{\ps_1,\ldots,\ps_p}))
} 
 &=& \SetTo{p}
 \\[\NL]
\multicolumn{1}{l}{
\EvalItems(\rits(\_,\pList{i_1\ldots,i_l},\pList{\ps_1,\ldots,\ps_l}))
} 
 &=& \Set{i_1\ldots,i_l}
 \\[\NL]
\multicolumn{1}{l}{
\EvalItems(\runIts(\_,\pList{i_1\ldots,i_l},\pList{\ps_1,\ldots,\ps_l}))
} 
 &=& \Set{i_1\ldots,i_l}
 \\[\NL]
%\multicolumn{1}{l}{
%\EvalItems(\rselIts(.,.,.,\pList{\ps_1,\ldots,\ps_n}))
%} 
% &=& P \cup N 
% \\[\NL]
\multicolumn{1}{l}{
\EvalProps(\rpattProps(\_,\pList{(k'_{i_1},p_{j_1}),\ldots,(k'_{i_l},p_{j_l})},\pList{\ps_1,\ldots,\ps_l}))
} %\\[\NL]
&=&
  \Set{k'_{i_1},\ldots,k'_{i_l}} 
 \\[\NL]
\multicolumn{1}{l}{
\EvalProps(\rprops(\_.,\pList{(k'_{i_1},k_{j_1}),\ldots,(k'_{i_l},k_{j_l})},\pList{\ps_1,\ldots,\ps_l}))
} %\\[\NL]
&=&
  \Set{k'_{i_1},\ldots,k'_{i_l}} 
 \\[\NL]
\multicolumn{1}{l}{
\EvalProps(\raddProps(\_,\pList{k_{i_1}\ldots,k_{i_l}},\pList{\ps_1,\ldots,\ps_l}))
} %\\[\NL]
&=&
  \Set{k_{i_1},\ldots,k_{i_l}} 
 \\[\NL]
\multicolumn{1}{l}{
\EvalProps(\runProps(\_,\pList{k_{i_1}\ldots,k_{i_l}},\pList{\ps_1,\ldots,\ps_l}))
} %\\[\NL]
&=&
  \Set{k_{i_1},\ldots,k_{i_l}} 
 \\[\NL]
\multicolumn{1}{l}{
\EvalItems(\rcont(\_,\pList{\ps_1,\ldots,\ps_l}))
} 
&=& \SetST{i}{r(\ps_i)=T} \\[\NL]
\EvalStar(\rany/\rall/\rone(\_,\pList{\ps_1,\ldots,\ps_n}))
                                              &=& \bigcup_{i\in\SetTo{n}}\EvalStar(\ps_i) \\[\NL]
%\EvalStar(\rall(\_,\pList{\ps_1,\ldots,\ps_n}))
%                                              &=& \bigcup_{i\in\SetTo{n}}\EvalStar(\ps_i) \\[\NL]
%\EvalStar(\rone(\_,\pList{\ps_1,\ldots,\ps_n}))
%                                              &=& \bigcup_{i\in\SetTo{n}}\EvalStar(\ps_i) \\[\NL]
\EvalStar(\rif/\rthen/\relse/\rnot(\_,\ps)) &=& \EvalStar(\ps) \\[\NL]
\EvalStar(\rdref/\rddref/\rddref\rkw{AsRef}(\_,\ps)) &=& \EvalStar(\ps) \\[\NL]
\EvalStar(\rdepS(\_,\pList{k_{i_1},\ldots k_{i_l}},\pList{\ps_1,\ldots,\ps_l})) &=& \bigcup_{i\in\SetTo{l}}\EvalStar(\ps_i) \\[\NL]
%\EvalStar(\rnot(\_,\ps)) &=& \EvalStar(\ps)    \\[\NL]
%\EvalStar(\atrue/\afalse) &=& \EmptySet \\[\NL]
\EvalStar(\rschema(C,J,S,T,\pList{\pk_1,\ldots,\pk_n}))  &=& \bigcup_{i\in\SetTo{n}}\EvalStar({\pk_i})  \\[\NL]
%\EvalStar(\rschema(C,J,S,F,\pList{\pk_1,\ldots,\pk_n}))  &=& \EmptySet  \\[\NL]
\EvalStar(\pk/\ps) &=& \emptyset \qquad\qquad \mbox{otherwise} \\[\NL]
%\end{array}
%$$
%
%$$\begin{array}{lllllllllllll}
\!\!\!\AdjEvalStar(\pk):\\[\NL]
\multicolumn{1}{l}{
\AdjEvalItems(\rprefIts(\_,\pList{\ps_1,\ldots,\ps_n}))
} 
 &=& \SetTo{p}
 \\[\NL]
 \multicolumn{1}{l}{
\AdjEvalProps(\rpattProps(\_,\pList{(k'_{i_1},p_{j_1}),\ldots,(k'_{i_l},p_{j_l})},\pList{\ps_1,\ldots,\ps_l}))
} %\\[\NL]
&=&
  \Set{k'_{i_1},\ldots,k'_{i_l}} 
 \\[\NL]
\multicolumn{1}{l}{
\AdjEvalProps(\rprops(\_,\pList{(k'_{i_1},k_{j_1}),\ldots,(k'_{i_l},k_{j_l})},\pList{\ps_1,\ldots,\ps_l}))
} %\\[\NL]
&=&
  \Set{k'_{i_1},\ldots,k'_{i_l}} 
 \\[\NL]
\multicolumn{1}{l}{
\AdjEvalStar(\pk)
} 
&=& \EmptySet \ \ \ \mbox{otherwise}
\end{array}
$$


==> schemabl.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "faz": 0}
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/failing_props_hidden_inside_anyOf.json",
  "type": "object",
  "anyOf": [ {"properties": { "faz": false }} ],
  "unevaluatedProperties": false 
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
	"valid": false,
	"keywordLocation": "https://formalize.edu/failing_props_hidden_inside_anyOf.json",
	"absoluteKeywordLocation": "",
	"instanceLocation": "",
	"errors": [
		{
			"valid": false,
			"error": "All anyOf failed: [[0 at #/faz failed against https://formalize.edu/failing_props_hidden_inside_anyOf.json#/anyOf/0/properties/faz with \"False\"]]",
			"keywordLocation": "https://formalize.edu/failing_props_hidden_inside_anyOf.json",
			"absoluteKeywordLocation": "",
			"instanceLocation": "#"
		},
		{
			"valid": false,
			"error": "False",
			"keywordLocation": "https://formalize.edu/failing_props_hidden_inside_anyOf.json#/unevaluatedProperties",
			"absoluteKeywordLocation": "#/unevaluatedProperties",
			"instanceLocation": "#/faz"
		}
	]
}
\end{lstlisting}
\end{querybox}

\caption{Schema vs keywords:Annotations returned by {\BL}, example \ref{ex:schema}.}
\label{fig:schemabl}
\end{figure}


==> schemaje.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "faz": 0}
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/failing_props_hidden_inside_anyOf.json",
  "type": "object",
  "anyOf": [ {"properties": { "faz": false }} ],
  "unevaluatedProperties": false 
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "valid": false,
  "keywordLocation": "",
  "absoluteKeywordLocation": "https://formalize.edu/failing_..._anyOf.json#",
  "instanceLocation": "",
  "errors": [
    {
      "valid": false,
      "keywordLocation": "/anyOf/0",
      "absoluteKeywordLocation": "https://formalize.edu/failing_..._anyOf.json#/anyOf/0",
      "instanceLocation": "",
      "errors": [
        {
          "valid": false,
          "keywordLocation": "/anyOf/0/properties/faz",
          "absoluteKeywordLocation": "https://formalize.edu/failing_..._anyOf.json#/anyOf/0/properties/faz",
          "instanceLocation": "/faz",
          "error": "All values fail against the false schema"
        }
      ]
    },
    {
      "valid": false,
      "keywordLocation": "/unevaluatedProperties",
      "absoluteKeywordLocation": "https://formalize.edu/failing_..._anyOf.json#/unevaluatedProperties",
      "instanceLocation": "/faz",
      "error": "All values fail against the false schema"
    }
  ]
}
\end{lstlisting}
\end{querybox}

\caption{Schema vs keywords:Annotations returned by json-everywhere, example \ref{ex:schema}.}
\label{fig:schemaje}
\end{figure}


==> schemajs.tex <==
\begin{figure}
\small
Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "faz": 0}
\end{lstlisting}
\end{querybox}

Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/failing_props_hidden_inside_anyOf.json",
  "type": "object",
  "anyOf": [ {"properties": { "faz": false }} ],
  "unevaluatedProperties": false 
}
\end{lstlisting}
\end{querybox}

Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
    "valid": false,
    "instanceLocation": "",
    "keywordLocation": "",
    "absoluteKeywordLocation": "https://formalize.edu/..._$defs.json#",
    "errors": [
        {
            "instanceLocation": "/faz",
            "keywordLocation": "/$ref/properties/faz",
            "absoluteKeywordLocation": "https://formalize.edu/..._$defs.json#/$defs/fazfalse/properties/faz",
            "error": "The instance is disallowed by a boolean false schema"
        },
        {
            "instanceLocation": "",
            "keywordLocation": "/unevaluatedProperties",
            "absoluteKeywordLocation": "https://formalize.edu/..._$defs.json#/unevaluatedProperties",
            "error": [
                "faz"
            ]
        }
    ]
}
\end{lstlisting}
\end{querybox}
\caption{Schema vs.\ keywords: Annotations returned by {\JSD}, example \ref{ex:schema}.}
\label{fig:schemajs}
\end{figure}


==> schemake.tex <==
\begin{figure}
\small

Instance:
\begin{querybox}{}
\begin{lstlisting}[style=querynonumbers]
{ "faz": 0 }
\end{lstlisting}
\end{querybox}


Schema:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "$id": "https://formalize.edu/failing_props_hidden_inside_anyOf.json",
  "type": "object",
  "anyOf": [ {"properties": { "faz": false }} ],
  "unevaluatedProperties": false 
}
\end{lstlisting}
\end{querybox}
 
Output:
\begin{querybox}{}
\begin{lstlisting}[style=query]
{
  "errors": [
    {
      "absoluteKeywordLocation": "https://formalize.edu/failing_props_hidden_inside_anyOf.json#/anyOf/0/properties/faz",
      "error": "property not permitted",
      "instanceLocation": "/faz",
      "keywordLocation": "/anyOf/0/properties/faz"
    },
    {
      "absoluteKeywordLocation": "https://formalize.edu/failing_props_hidden_inside_anyOf.json#/unevaluatedProperties",
      "error": "additional property not permitted",
      "instanceLocation": "/faz",
      "keywordLocation": "/unevaluatedProperties"
    },
    {
      "absoluteKeywordLocation": "https://formalize.edu/failing_props_hidden_inside_anyOf.json#/unevaluatedProperties",
      "error": "not all additional properties are valid",
      "instanceLocation": "",
      "keywordLocation": "/unevaluatedProperties"
    }
  ],
  "valid": false
}
\end{lstlisting}
\end{querybox}

\caption{Schema vs keywords:Annotations returned by {\KE}, example \ref{ex:schema}.}
\label{fig:schemaje}
\end{figure}

